Domain-Agnostic Hardware Fingerprinting-Based Device Identifier for Zero-Trust IoT Security

Next-generation networks aim for comprehensive connectivity, interconnecting humans, machines, devices, and systems seamlessly. This interconnectivity raises concerns about privacy and security, given the potential network-wide impact of a single compromise. To address this challenge, the Zero Trust (ZT) paradigm emerges as a key method for safeguarding network integrity and data confidentiality. This work introduces EPS-CNN, a novel deep-learning-based wireless device identification framework designed to serve as the device authentication layer within the ZT architecture, with a focus on resource-constrained IoT devices. At the core of EPS-CNN, a Convolutional Neural Network (CNN) is utilized to generate the device identity from a unique RF signal representation, known as the Double-Sided Envelope Power Spectrum (EPS), which effectively captures the device-specific hardware characteristics while ignoring device-unrelated information. Experimental evaluations show that the proposed framework achieves over 99%, 93%, and 95% testing accuracy when tested in same-domain (day, location, and channel), cross-day, and cross-location scenarios, respectively. Our findings demonstrate the superiority of the proposed framework in enhancing the accuracy, robustness, and adaptability of deep learning-based methods, thus offering a pioneering solution for enabling ZT IoT device identification.

==> 7-performance.tex <==

\begin{figure}
     \subfloat[15 Pycom transmitting devices\label{tx}]{%
       \includegraphics[width=0.23\textwidth, height = 0.2\textwidth]{Figures/Dataset/tx_pic.png}
     }
    \hspace{0.00001cm}
     \subfloat[Location Setup\label{loc_setup}]{%
       \includegraphics[width=0.23\textwidth, height = 0.2\textwidth]{Figures/Dataset/loc_fixed.PNG}
     }
     \caption{IoT Testbed consisting of 15 Pycom transmitting devices and a USRP B210 receiving device}
     \label{testbed}
\end{figure}



To assess the effectiveness of \framework,
%in generating strong identities for IoT devices and verifying their identities across domains, 
we leveraged our 15-Pycom-device testbed, shown in Fig.~\ref{tx}, to generate and collect WiFi 802.11b datasets for the following three scenarios: 
\begin{itemize}
\item {\bf Fixed-location scenario:} Devices were placed in three different fixed locations, namely Loc A, Loc B, and Loc C, as depicted in Fig.~\ref{loc_setup}.

\item {\bf Random-location scenario:} Devices were placed randomly within $3$-meter distances from the USRP receiver.

\item {\bf Cross-day wireless scenario:} Data was collected in an indoor wireless scenario over three consecutive days.  
\end{itemize}
%
In our evaluation, we employed two key performance metrics: same-domain accuracy and cross-domain accuracy. Same-domain accuracy measures the ability of the device identifier to identify devices accurately when the testing data/packets are drawn from the same training domain. On the other hand, cross-domain accuracy evaluates the models' ability to generalize across different domains, such as different locations, channels, or days. To ensure robust results, we utilized the 5-fold cross-validation technique, dividing each device's data into five non-overlapping partitions of equal size. We evaluated the performance of our proposed \framework~and \hl{compared it with the same CNN framework fed with a typical IQ representation as an input (referred to as IQ-CNN)}. %and compared it with the same CNN framework but when fed with a typical I/Q representation as an input (referred to as IQ-CNN). %We employed the 5-fold cross-validation method, where each device's data is divided into five non-overlapping, equally-sized partitions. In each fold of cross-validation, we used four partitions for training (3200 packets) and the remaining partition for testing (800 packets). We then averaged the results obtained from each fold to produce a final estimate of the model's performance. 
%For the \proposed~input, we represented each packet by a 2x4096 tensor, which encapsulates the \proposed~representation of both the I and Q components. %In contrast, for I/Q input, we represented each packet using a 2x8192 tensor, comprising the first 8192 samples of both the I and Q components as this window size provides the best performance for the I/Q representation input.




\subsection{Device Identification Results}
\subsubsection{Robustness to Location Changes with Fixed Placement}\label{subsub:fix-loc}

\begin{figure*}
\centering
 \includegraphics[width=\linewidth]{Figures/results/EPS-results.pdf}
 \caption{\framework~performance: the testing accuracies under the location and time scenarios} %
\label{eps-locations}
\end{figure*}

% \begin{figure}
% \centering
%     %\subfloat[Testing accuracy]{
%    \includegraphics[width=\columnwidth]{Figures/results/eval_locations.pdf}
%  \caption{EPS-CNN Vs. IQ-CNN performance: Location Scenarios} %
% \label{eps-locations}
% \end{figure}


We evaluate our proposed \framework~framework using the WiFi dataset captured at three different locations %, as described in Sec.~\ref{location_Setup}, 
to assess its robustness to changes in device locations. Fig.~\ref{eps-locations} displays the results for \framework, where LocA, LocB, and LocC represent transmitter distances of 1m, 2m, and 3m from the USRP receiver.

The \framework~framework demonstrates remarkable device identification effectiveness, achieving exceptional same-location testing accuracies at all locations. Specifically, the average same-location testing identification accuracies at Locations A, B, and C are 100\%, 99.6\%, and 96.7\%, respectively. Moreover, \framework~excels in cross-location evaluation, maintaining high performances with average testing identification accuracies of 91.3\% and 95.5\% when trained on location A and tested on locations B and C, respectively. Similar impressive results are seen when trained on locations B and C and tested on the other locations. In \hl{Fig.}~\ref{eps-locations}, \hl{panels (a,b,c) illustrate the superiority of our \framework~framework compared to the conventional IQ-CNN framework in the cross-location scenario.} 
 
To the best of our knowledge, this is the highest performance achieved by a DL-based device fingerprinting method when the learning models are tested and trained on different domains. 

%Note the significant accuracy difference between that achieved by the proposed \framework~and that achieved by the conventional IQ-CNN across the three scenarios (i.e., a drop from 90+\% to as low as 25\%).
%The confusion matrices in Figs.~\ref{IQ-loc1}, \ref{IQ-loc2}, \ref{IQ-loc3} show the struggle of the trained model to correctly classify the devices when the corresponding packets are captured in a different location. 
%The results clearly demonstrate the superiority of the \proposed-based deep learning framework in device fingerprinting, particularly in cross-domain evaluations. 


\subsubsection{Robustness to Location Changes with Random Placement}\label{subsub:ran-loc}



We also considered evaluating the effectiveness of \framework~under two random-location setups. %For each setup, during training (referred to as enrolment), all devices transmit from a fixed location, 1m away from the receiver; and during testing (referred to as deployment), the devices transmit from random locations all within 3m from the receive.
%
% The \framework~framework exhibits strong performance in both same-domain and cross-domain evaluations under random-location setups.
Fig.~\ref{eps-locations}d \hl{shows that \framework~achieves high average cross-domain testing accuracies of 93\% and 98\%, respectively, when trained on Location A and tested under random-location setups 1 and 2. In contrast, IQ-CNN's performance deteriorates when it is tested on random placement. The average testing accuracies of IQ-CNN are 40\% and 58\% under random-location setups 1 and 2, respectively.} 
%Notably, Fig.~\ref{eps-rand1}, showing the confusion matrix under random-location setup 2, showcases the framework's exceptional classification accuracy for most devices. 
%In contrast, the IQ-based model (IQ-CNN) experiences significant performance degradation on both random-location setups, with cross-domain testing accuracies of only 40.2\% and 58.2\% on setups 1 and 2, respectively. Through the confusion matrix, Fig.~\ref{iq-rand1} provides a clear depiction of the IQ-CNN framework's struggle in recognizing devices when randomly deployed around the receiver. 

 




 \subsubsection{Robustness to Time Changes}




 The proposed \framework~framework was also evaluated on a cross-day scenario using the indoor wireless WiFi dataset collected over three consecutive days. Fig.~\ref{eps-locations}e presents the average testing accuracy of \framework~when trained on one day and tested on one of the other three days. \hl{The same-day testing accuracies (both training data and testing data are collected on the same day) were found to be 100\%.
  
 More interestingly, for the cross-day evaluation, our experiments show that \framework~maintains remarkable accuracy when tested on a different day, as demonstrated in Fig}.~\ref{eps-locations}e. \hl{Specifically, when the learning model is trained on day 1 data but tested on data collected on a different day, the average cross-domain testing accuracies of the \framework~are 93\% (compared to 88\%, IQ-CNN) and 92\% (compared to 89\%, IQ-CNN) when tested on day 2 and day 3 data, respectively, as shown in Fig}.~\ref{eps-locations}e. Similar impressive results are obtained when trained on days 2 and 3 and tested on the other days.
\subsection{Further Analysis}
\hl{In addition to providing enhanced security, the \framework~preserves privacy by minimizing the transmission of device credential information during network access operations. Moreover, it eliminates the need for error-prone manual upkeep of MAC Authentication Bypass/allow lists, as security policy rule recommendations are automatically derived from the \framework's output.

The durability of our framework inherently depends on the aging rate of hardware components, especially the quality of the crystal oscillator, and the intra-distance between different fingerprints in the latent space. Consequently, it varies between deployments. In our current evaluation, we have concentrated on showcasing the resilience of our framework against short-term aging, a standard practice in the assessment of newly proposed device fingerprinting techniques. This short-term analysis, conducted over a week, forms a robust foundation for understanding initial performance. However, we acknowledge the necessity to explore the model's behavior under prolonged aging circumstances, spanning months or even years, aligning with the typical lifespan of IoT devices.} %Once the durability at a specific deployment is determined, continuous fine-tuning or retraining is recommended to adapt to evolving characteristics introduced by aging. This iterative process ensures the adaptability and robustness of our framework over time. }
   

